Informatiekunde -- Curriculum 2003

This document discusses the curriculum of the business informatics program of the Nijmegen Institute for Informatics and business informatics (NIII). The aim is to provide a 'repository' with regard to the structure of the curriculum, which will apply from 2003. In the past three years, the image of information science as a discipline has been further concretised at both national and Nijmegen level. Curriculum 2003 is on the one hand the result of this concretization and on the other hand of the three years of experience that has now been built up within the NIII with the information science training. In this document, therefore, explicit attention will also be paid to the 'migration' from the existing 'start-up' curricula: 2000, 2001 and 2002. It should be noted here that the students of cohort 2000 will in principle have completed the bachelor's phase of the program this year (2003). Complete information science education. No specific `migration 'is therefore necessary for this group of students.

==> GG <==
Tot de grondslagen van de informatiekunde rekenen we de volgende gebieden:
\begin{itemize}
  \item Systeemtheorie
  \item Informatietheorie
  \item Communicatietheorie
\end{itemize}
Met betrekking tot de grondslagen van de informatiekunde, is een
informatiekundige na afloop van de studie in staat om:
\begin{description}
   \item[Redeneren over grondslagen --] ... te redeneren over de grondslagen
   van de informatiekunde;
   \item[Grondslagen toepassen --] ... in staat om de bij de grondslagen
   behorende methoden, technieken en theorie\"en toe te passen in concrete
   situaties;
\end{description}
\def\B{Belangstellend} \def\U{Uitvoerend} \def\R{Richtinggevend} \def\K{Kaderzettend}
Wanneer we deze vaardigheden vervolgens koppelen aan ambitieniveau's, dan leidt
dit tot de volgende tabel:
\begin{center} \footnotesize
     \begin{tabular}{l|l|l|l|l|l}
     Vaardigheid                & Propedeuse & Bachelor & Master & Post Graduate & Profiel\\
     \hline
%%%%
     \hline
                                &            &          &        & \K           & Onderzoeker\\
     \cline{5-6}
     Redeneren over grondslagen & \B         & \U       & \R     & \K           & Docent\\
     \cline{5-6}
                                &            &          &        & \K           & Professional\\
     \hline
%%%%
     \hline
                                &            &          &        & \K           & Onderzoeker\\
     \cline{5-6}
     Grondslagen toepassen      & \B         & \U       & \R     & \K           & Docent\\
     \cline{5-6}
                                &            &          &        & \K           & Professional\\
     \hline
  \end{tabular}
\end{center}


==> pub.tex <==
{\sc Published as:}
\begin{quote}
  V.~{Kamphuis}, H.A.~(Erik) {Proper}, and S.J.B.A. {Hoppenbrouwers}. {\em {Informatiekunde 2003 -- Curriculum}}. Nijmegen Institute for Information and Computing Sciences, University of Nijmegen, Nijmegen, The Netherlands, EU, 2003. In Dutch.
\end{quote}


==> tmp <==
\long\def\ExternVak#1#2#3#4#5{
  \par
  \begin{minipage}{\textwidth}
     \hrule
     \vspace{0.5em}
     \section{#1}
     \vspace{-0.4em}
     \hrule
   
     \vspace{0.2em}
     \noindent \tabcolsep=0pt
     \begin{tabular}{ll}
        {\bf Omvang:}         & #2\\
   	{\bf Afdeling:}       & Extern\\
        {\bf Geroosterd in:~} & #4\\
        {\bf Semester:}       & #3\\
     \end{tabular}\\
     {\bf Opties:}
     \begin{itemize}
        #5
     \end{itemize}
     \hrule
  \end{minipage}

  \vspace{1cm}
}


==> voorpagina-doelen.tex <==
\begin{titlepage}

\href{http://www.niii.kun.nl}{
{\ExtraHuge \NIIITekst} 
\begin{tabular}[b]{l}
 \Large \sf nijmeegs instituut\\[0.2mm]
 \Large \sf voor informatica en informatiekunde
\end{tabular}}

\begin{center}
  \vfill

  \vfill

  \textcolor{blue}{\ExtraHuge Informatiekunde}
 
  \vspace{0.5cm}

  \textcolor{red}{\Huge Doelstellingen \& Eindtermen}

  \vfill

  \Image{width=7cm}{DaVinci}

  \vfill
\end{center}

\textcolor{blue}{\input{one-liner}}

%\begin{center}
%  \textcolor{red}{\large Versie van: \today}
%\end{center}

\end{titlepage}

